Hierarchical Graph Neural Networks for Causal Discovery and Root Cause Localization

In this paper, we propose REASON, a novel framework that enables the automatic discovery of both intra-level (i.e., within-network) and inter-level (i.e., across-network) causal relationships for root cause localization. REASON consists of Topological Causal Discovery and Individual Causal Discovery. The Topological Causal Discovery component aims to model the fault propagation in order to trace back to the root causes. To achieve this, we propose novel hierarchical graph neural networks to construct interdependent causal networks by modeling both intra-level and inter-level non-linear causal relations. Based on the learned interdependent causal networks, we then leverage random walks with restarts to model the network propagation of a system fault. The Individual Causal Discovery component focuses on capturing abrupt change patterns of a single system entity. This component examines the temporal patterns of each entity's metric data (i.e., time series), and estimates its likelihood of being a root cause based on the Extreme Value theory. Combining the topological and individual causal scores, the top K system entities are identified as root causes. Extensive experiments on three real-world datasets with case studies demonstrate the effectiveness and superiority of the proposed framework.

==> abstract.tex <==
\begin{abstract} 
Root cause analysis aims to locate the root causes of system failures by analyzing the metrics data of monitoring systems. 
It is indispensable for maintaining the stability and robustness of large-scale complex systems.
Existing methods mainly focus on identifying the root causes on a single isolated network, while many %real-world complex systems exhibit interdependent networks structures
real-world systems are complex and exhibit interdependent structures (\textit{i.e.}, multiple networks of a system %interconnect with one another
are interconnected by cross-network links). In interdependent networks, the malfunctioning patterns of problematic system entities can propagate %from one network to another.
across different networks or different levels of system entities. Thus, ignoring the %interdependent networks structure will result in suboptimal root cause analysis results. 
interdependency inevitably results in suboptimal root cause analysis results.

In this work, we propose \model, an interdependent causal networks based framework, to enable the automatic discovery of both intra-level (\textit{i.e.}, within-network) and inter-level (\textit{i.e.}, across-network) causal relationships for root cause localization. 
The \model\ framework consists of Topological Causal Discovery and Individual Causal Discovery.
The Topological Causal Discovery component %model
aims to %capture
model the fault propagation %patterns
for tracing back root causes. %localization.
To %achieve this goal,
this end, we %first
propose novel hierarchical graph neural networks to construct the interdependent causal networks
by modeling both intra-level and inter-level non-linear causal relations. Based on the learned interdependent causal networks, we then leverage random walk with restarts to model the network propagation of a system fault. The Individual Causal Discovery component %model
focuses on individual causal effects, by analyzing each system entity's metric data (\textit{i.e.}, time series) with the underlying hypothesis that the metric data of the root causes often fluctuates more strongly than those of other system entities during the incidence 
of system faults. %Individual Causal Discovery model 
This component examines the temporal patterns of each entity's metric data, 
and estimates its likelihood of being a root cause based on the Extreme Value theory. 
Combining the %individual and topological
topological and individual causal scores, root causes are detected as the top $K$ system entities.
Extensive experiments on three real-world datasets with case studies demonstrate the effectiveness and superiority of the proposed framework.
\end{abstract}

==> introduction.tex <==
\section{Introduction} 
Root Cause Analysis (RCA) refers to the process of identifying the root causes of system faults  using surveillance metrics data~\cite{andersen2006root,kiciman2005root}.
\nop{There are numerous complicated real-world systems that play crucial roles in maintaining the normal functioning of civilization.}
It has been widely used in IT operations, industrial process control, telecommunications, {\em etc.}, because a failure or malfunction in these systems would significantly degrade 
user experiences and cause 
business losses.
For instance, an intermittent outage of Amazon Web Services %resulted
can result in %approximately
around \$210 millions loss~\cite{amazon}.
To maintain the reliability and robustness of such systems, the system's Key Performance Indicators (KPIs), such as latency or connection time in a microservice system, and metrics data, such as CPU/memory usages in a microservice system are often monitored and recorded %logged
in real-time for system diagnosis.
Nevertheless, the big size of %the
monitoring data and the complexity of such systems make manual detection of root causes prohibitively costly %manually identifying root causes is time-consuming, labor-intensive,
and error-prone. %needs extensive domain expertise.
%Thus, it is indispensable for these large and distributed systems to automatically identify the root causes of system failures by analyzing vast amounts of monitoring data.
%Therefore,
As such, an efficient and effective root cause analysis that %, which
enables %speedy
fast service recovery and loss mitigation, becomes %very important
crucial for %maintaining the stability and robustness of
stable running and robust management of large-scale complex systems.

%RCA has received considerable research interest in recent years ~\cite{jurn2018survey,7069265,fourlas2021survey}.
%Although existing works have achieved good performance, the following issues still limit their practicality and effectiveness.

% \begin{figure}[htbp]
% \vspace{-0.1cm}
% \centering
% \subfigure[Precision@K for Swat]{
% \includegraphics[width=4.1cm]{img/micro-service.pdf}
% }

% % \hspace{-3mm}
% % \vspace{-4mm}
% \subfigure[Precision@K for WADI]{
% \includegraphics[width=4.1cm]{img/system_fault.pdf}
% }

% % \vspace{-0.5cm}
% \caption{Study of the necessity for integrating individual and topological causal analysis results.}
% \label{fig:mcs}
% % \vspace{-0.3cm}
% \end{figure}

\begin{figure}[!t]
% \vspace{-20pt}
    \centering
    \includegraphics[width=0.75\linewidth]{img/mcs.pdf}
    % \vspace{-0.2cm}
    \captionsetup{justification=justified, singlelinecheck=off}
    % \vspace{-0.33cm}
    \caption{ An example of interdependent causal networks. The main network is represented (\textit{i.e.}, server/machine network) by dashed nodes and edges. The domain-specific networks (\textit{i.e.}, application/pod networks) are represented by solid nodes and edges. The edges highlighted by red colors indicate how the malfunctioning effects of a root cause (\textit{i.e.}, Django-search) propagate in the system. 
    }
    % \vspace{-0.22cm}
    \label{fig:mcs}
        % \vspace{-5pt}
\end{figure}

%Although the recent years have witnessed
%Despite the significant progress of the root cause analysis techniques recently~\cite{jurn2018survey,7069265,fourlas2021survey}, %the practicality and efficacy of root cause analysis are limited by two major factors: 

Previous research on root cause analysis~\cite{liu2021microhecl,lin2018microscope,9521340,meng2020localizing}  %has been limited to an idealized case,
mostly limit their focus to a simplified case, where the target system is modeled as a single isolated causal network or graph, %\footnote{In this paper, we use network and graph interchangeably}, 
and the system malfunctioning effects %behavior can
can only propagate within the same network of entities. %behavior can
For instance, Liu \textit{et al.}~\cite{liu2021microhecl} generated a service call graph based on domain-specific software and rules to identify different kinds of service root causes. 
Chen \textit{et al.}~\cite{lin2018microscope} constructed a directed acyclic graph that depicts the invoking relations among microservice applications for locating root causes. These methods have shown promising results on the systems with isolated network structures.    

However, a real-world complex system usually consists of multiple networks that coordinate %work together
in a highly complex %and coordinated
manner~\cite{gao2014single,amini2020interdependent,gao2012networks}. These networks interact with each other, %one another,
and the failure of a system entity in one network could %lead to the failure of
spread to the dependent entities in other networks, which in turn may result in %cause further damage to the first level, leading to cascading failures
cascading damages/failures~\cite{buldyrev2010catastrophic,ash2007optimizing,liu2016breakdown} that could circulate the interconnected levels, %and possible
with catastrophic consequences. For instance, Figure~\ref{fig:mcs} shows the malfunction of the pod \textit{Django-search} first spreads to the server network and causes the fault of the server \textit{Compute-1}; Then, the malfunctioning effects spread to the pod network of \textit{Compute-2} and causes the faults of the pod \textit{Mongodb} and \textit{Mysql}; Finally, the pod \textit{Sdn} in \textit{Infra-1} is also affected, resulting in the system failure. In this failure case, if we only model the server network (\textit{i.e.}, the three servers) or one of the three pod networks of the microservice system, it is very hard to pinpoint %accurately identify
the root cause \textit{Django-search}. In contrast, %Thus,
modeling the interconnected multi-network structures %can help
%is vital for
provides a comprehensive understanding of the %a
system %understand a system’s robustness
and %enables design of
a more effective root cause analysis. 
%\begin{itemize}

\nop{\item \textbf{ \st{Issue 1: \st{requiring} excessive domain knowledge.} } 
{\color{red} Yanjie: every practical method needs domain knowledge. It is not a unique and articulate issue. maybe change your wording. }
For instance, Li \textit{et al.} located root cause via tracing on predefined invocation relations among different  microservices~\cite{9521340}. %And
Liu \textit{et al.} identified different kinds of service anomalies using a service call graph generated by domain-specific software and rules~\cite{liu2021microhecl}.
These methods rely heavily on domain knowledge for detecting root causes. %to identify root causes effectively.
%In fact, however,
However, for many complex systems, it is expensive %impracticable
to acquire accurate domain knowledge, %from many real-world complex systems. %lack domain knowledge.
%Thus, the methods that require domain knowledge
which makes these methods %are
difficult to generalize to different domains. %other fields. %this characteristic makes such approaches insufficiently generic.
{\color{red} Yanjie: lacks a summary of this issue, dont just list a bunch of papers. }

\textbf{Issue 2: \st{ignoring} hierarchical structures.}
\nop{For example, Meng \textit{et al.} first discovered the causal relations among different time series, then utilized random walk to locate root cause metrics in a microservice~\cite{meng2020localizing}. 
Deng \textit{et al.} proposed an attention-based graph neural network to detect correlations among sensors and utilized attention scores to identify root causes in water treatment networks~\cite{deng2021graph}.
The structure learning part of these approaches is simple and ignores hierarchies in complex systems, which limits their effectiveness.}
Real-world complex systems usually
consist of different levels/layers of entities that coordinate %work together
in a highly complex %and coordinated
manner. One example is the cloud computing facilities with microservice architecture (see Figure~\ref{fig:mcs}), which is typically constituted by %consist of
hundreds of different levels of entities that vary from servers to application software. %{\em etc.}
Previous researches~\cite{meng2020localizing,deng2021graph} %has been limited to an idealized case,
mostly limit their focus to a simplified case, where the fault patterns %behavior can
only propagate within %between
the same level of entities, %system components, but in real-world complex systems,
ignoring the fact that the failure of a entity in one level could lead to the failure of the dependent entities in other levels, which in turn may result in %cause further damage to the first level, leading to cascading failures
cascading damages that could circulate the interconnected levels, %and possible
with catastrophic consequences. For instance, Figure~\ref{fig:mcs} shows the malfunction of a pod causes the fault of a server machine, then the damaging effects spread to the whole system, resulting in the system failure. Thus, modeling the hierarchical structures %can help
is vital for a comprehensive understanding of a system %understand a system’s robustness
and %enables design of
a more effective root cause analysis framework.
%\end{itemize}
}
\nop{However, real-world complex systems (e.g. urban systems,  industrial systems, and microservice systems) are replete with hierarchical graph structures that are crucial for identifying root causes.
For instance, Figure ~\ref{fig:mcs} shows a root cause example in a microservice system, in which the malfunction of a pod causes the anomaly of a server machine, then the damaging effects spread to the whole system, resulting in the system failure.
But how to model such complex structural information in systems for root cause localization?}

\nop{Interdependent networks have been demonstrated to be an effective tool for modeling complex real-world systems across several disciplines, such as ranking, clustering, searching ~\cite{ni2014inside,}. 
In light of these impressive achievements, we adopt this graph data model to capture complex topological causal relations in real-world systems for localizing root causes.
To the best of our knowledge, we are the first to introduce this concept into the RCA domain.}



Recently, a %very
promising approach %means
for modeling such interconnected structures in complex systems has emerged through
the concept of interdependent networks (or network of networks)~\cite{buldyrev2010catastrophic,liu2016breakdown,amini2019sustainable,gao2014single,NEKOVEE2007457,gao2012networks,ni2014inside,amini2020interdependent}. In interdependent networks, each node of the main network can be represented as another network. Let us elaborate using the example in Figure~\ref{fig:mcs} again. Here, the dashed network represents a server/machine network (the main network), where the nodes are three different servers and edges/links indicate the causal relations among different servers. Each node of this main network is further represented as a pod network (the domain-specific network), where nodes are pods and edges denote their causal relations. Collectively, we call this structure a (server-pod) interdependent networks. And since all the edges in this interdependent networks indicate causal dependencies, we further call it \textit{interdependent causal networks}.\nop{the nodes \st{within}  one network are connected by \st{connectivity links} {\color{red} Yanjie: what are connectivity links?} (\textit{e.g.}, the friendships between individuals in a social network), and the nodes of different networks are adjacent to one another via \st{dependency links} {\color{red} Yanjie: you need to introduce this concept earlier, some descriptions are confusing. } (\textit{e.g.}(\textit{e.g.}, employer-employee relationships in a social network). }
Interdependent networks have been widely used in the study of various topics, including the spreading of an epidemic~\cite{saumell2012epidemic}, the academic influence of scholars~\cite{ni2014inside}, and the spreading pattern of rumors in the complex social network~\cite{NEKOVEE2007457}. However, existing methods only consider physical or statistical correlations, but not causation, and thus cannot be directly applied %to localizing
for locating root causes.

Enlightened by the interdependent networks, %the aim of
this paper %is
aims to learn interdependent causal relationships in multi-network systems for accurately locating root causes when a system failure/fault occurs. Formally, given the system KPI data, the multi-level interconnected system entities, and their metrics data ({\em i.e.}, time series), %how can
we want to learn interdependent causal structures %from the monitoring data
for locating root causes of system failures, especially cascading failures~\cite{buldyrev2010catastrophic}. There are two major challenges in this task: %for achieving this:

\begin{itemize}
	\item \textbf{Challenge 1: Learning interdependent causal networks and modeling fault propagation in interdependent causal networks.}
	As aforementioned, in real-world systems with interdependent networks structures, malfunctioning effects of root causes can propagate to other nodes of the same level or different levels (\textit{i.e.}, main network level and domain-specific network level), resulting in catastrophic failure in the whole system. To capture such propagation patterns for root cause localization, we need to learn the causal relationships not only within the same level but also across %cross
	levels. After modeling the interdependent causal relationships, we still need to model the propagation of malfunctioning effects in the learned causal interdependent networks.  %learn interdependent causal networks for building robust causal linkages between system entitis and system KPI.
	
	\item \textbf{Challenge 2: Capturing temporal patterns from the metrics data of individual system entity.} 
	In addition to the topological patterns, the features or metrics data, which are typically time series, associated with the %root
	system entities can also exhibit some abnormal %temporal
	patterns from temporal perspective during the incidence of system faults. For instance, the metrics of root causes typically fluctuate more strongly than those of other entities. Thus, the temporal patterns from the metrics  of each system entity can provide individual causal insights for locating root causes. The challenge is how to capture temporal patterns from each system entity and determine the individual causal effect corresponding to the system failure. 
	
\end{itemize}
 
\nop{There are two research challenges in this paper: \textit{(i) How to learn interdependent networks from monitoring entity metrics without massive domain knowledge?}
\textit{(ii) How to localize root causes based on learned causal structures for system failures?}}

To address these %aforementioned two
challenges, in this paper, we propose \model, a generic inte\underline{r}depend\underline{e}nt c\underline{a}u\underline{s}al networks based framework, for root cause l\underline{o}calizatio\underline{n} in complex systems with interdependent network structures.
\model\ consists of Topological Causal Discovery (TCD) and Individual Causal Discovery (ICD). 
For the TCD component, the assumption is that the malfunctioning effects of root causes can propagate to other system entities of the same level or different levels over time~\cite{buldyrev2010catastrophic,ash2007optimizing,liu2016breakdown}. To capture such propagation patterns, we first propose a hierarchical graph neural networks based causal discovery method to discover both intra-level (\textit{i.e.}, within-network) and inter-level (\textit{i.e.}, across-network) non-linear causal relationships.
Then, we leverage random walk with restarts to model the network
propagation of a system fault. 
%TCD aims to model the topological causal effects. %by learning interdependent causal networks and capturing fault propagation patterns. %that depict interdependent causal links from low-level nodes to high-level nodes to the system key performance indicator (KPI).
%The learning process for causal interdependent networks can be divided into intra-layer learning and inter-layer learning. 
%Specifically, for intra-layer learning, we build causal structures among different nodes at the same level based on the VAR model.
%During the learning process, graph neural networks are used to learn more robust non-linear causal relations through the message passing mechanism. We apply the same learning strategy for different level nodes.
\nop{To encode the non-linear causal relationships, graph neural networks (GNNs) are used to learn the representations of system entitis via the message passing mechanism. For inter-layer learning, we adaptively combine low-layer information into high-level nodes to influence the causal learning process at the high-level. In this way, we construct the whole causal interdependent graphs that describe the causal links from low-level nodes to high-level nodes to system KPI. Considering the fact that the negative impacts of root causes can spread to neighboring nodes until system failures, we employ the network propagation mechanism to simulate the fault propagation process in order to infer real root causes. Specifically, we first reverse the direction of learned interdependent causal graphs. Then, we regard the KPI node as the start point, and apply a random walk with restart algorithm to visit the learned interdependent graphs and record the visiting possibility of each node. Such probability scores are regarded as the topological causal scores. }%For the individual causal analysis, we investigate the temporal pattern of the system metric of nodes (i.e. system components) in isolation. 
The ICD component, on the other hand, focuses on individual causal effects, by analyzing the metrics data (\textit{i.e.}, time series) of each system entity.
%The underlying hypothesis behind ICA is that the time series of the root cause fluctuates significantly during system failures.
The underlying hypothesis behind ICD is that the metrics data of the
root causes often fluctuate more strongly than those of other system
entities during the incidence of system faults. We design an Extreme Value %extreme value
theory based method to capture the temporal fluctuation patterns and estimate the likelihood of each entity to be a root cause. %After the process, each node is associated with one individual causal score. 
Finally, we integrate the findings of the individual and topological causal discovery, and output the system entities with the top-$K$ greatest causal scores as the root causes.

\begin{figure*}[!t]
% \vspace{-15pt}
    \centering
    \includegraphics[width=0.92\linewidth]{img/Framework.pdf}
    % \vspace{-0.2cm}
    \captionsetup{justification=justified, singlelinecheck=off}
    % \vspace{-0.33cm}
    \caption{The overview of the proposed framework \model. It consists of three major steps: topological causal discovery, individual causal discovery, and causal integration.\nop{This framework locates root causes based on monitoring entity metrics and system KPI.
    Individual causal discovery is to capture fluctuation patterns of root causes. 
    Topological causal discovery is to capture the propagation characteristics of root causes.
    Causal integration integrates the discovery results of the two branches for locating root causes accurately.}
    }
    \vspace{-0.45cm}
    \label{fig:framework}
\end{figure*}


The %main
contributions of this work are summarized as follows:
\begin{itemize}
    %\item %We identify the importance of interdependent structures in root cause analysis for multi-level systems empirically.
    \item We identify an important and challenging problem of root cause localization in complex systems with interdependent network structures. 
    \item We introduce a novel and generic interdependent causal network based framework \model, covering both topological propagation patterns and individual temporal patterns, to accurately locate the root causes of system failures, especially cascading failures. To the best of our knowledge, \model\ describes the first attempt to incorporate interdependent networks for %with
    the root cause localization and causal discovery tasks. %that can be easily applied in real scenarios without domain knowledge.
    %\item We first introduce interdependent networks to formulate complex systems in the RCA domain and prove their effectiveness.
    \item We propose a novel hierarchical graph neural networks %network
    based method for detecting both intra-level (\textit{i.e.}, within-network) and inter-level (\textit{i.e.}, across-network) non-linear causal relationships on interdependent networks, and present a random walk based method for modeling the fault propagation in interdependent causal networks.
    \item We introduce an Extreme Value %extreme value
    theory based approach for modeling the temporal fluctuation patterns for individual causal discovery.   
    \item We conduct extensive experiments on three real-world datasets with case studies to validate the effectiveness of the proposed framework. 
\end{itemize}




















